M-STAR: Multi-Scale Spatiotemporal Autoregression for Human Mobility Modeling

Modeling human mobility is vital for extensive applications such as transportation planning and epidemic modeling. With the rise of the Artificial Intelligence Generated Content (AIGC) paradigm, recent works explore synthetic trajectory generation using autoregressive and diffusion models. While these methods show promise for generating single-day trajectories, they remain limited by inefficiencies in long-term generation (e.g., weekly trajectories) and a lack of explicit spatiotemporal multi-scale modeling. This study proposes Multi-Scale Spatio-Temporal AutoRegression (M-STAR), a new framework that generates long-term trajectories through a coarse-to-fine spatiotemporal prediction process. M-STAR combines a Multi-scale Spatiotemporal Tokenizer that encodes hierarchical mobility patterns with a Transformer-based decoder for next-scale autoregressive prediction. Experiments on two real-world datasets show that M-STAR outperforms existing methods in fidelity and significantly improves generation speed. The data and codes are available at https://github.com/YuxiaoLuo0013/M-STAR.

==> Table/alg.tex <==
\begin{algorithm}[htb]
    \caption{Multi-scale VQ-VAE Encoding via MST-Tokenizer}
    \label{alg:MST-Tokenizer}
    \SetKwInOut{KwData}{Inputs}
    \SetKwInOut{KwIn}{Hparams}
    \SetKwInOut{KwResult}{Return}
    \KwData{Trajectory $\mathcal{J}$}
    \KwIn{Number of scales $K$, spatial scales $\{s_k\}_{k=1}^{K}$, temporal scales $\{\tau_k\}_{k=1}^{K}$, codebook $\mathcal{Q}$}
    
    $\boldsymbol{R} \gets \emptyset$\; % \tcp*{Initialize residual token queue}
    
    \For{$k = 1$ \KwTo $K$}{
        $\mathbf{L}_k \gets \text{onehot}( \text{grid\_assign}(\mathcal{J}, s_k))$\; % \tcp*{Assign to spatial grids}
        $\mathbf{X}_k \gets \mathbf{L}_k \cdot E_k$\; % \tcp*{Spatial embedding}
        $\mathbf{Z}_k^{\text{enc}} \gets \operatorname{Interpolate}(\operatorname{TrajEncoder}(\mathbf{X}_k), \tau_k)$\; % \tcp*{Temporal encoding}
        
        \If{$k == 1$}{
            $\mathbf{F}_1^{\text{enc}} \gets \mathbf{Z}_1^{\text{enc}}$\; % \tcp*{Initial residual}
        }
        \Else{
            $\tilde{\mathbf{Z}}_k \gets \operatorname{Interpolate}(\mathbf{Z}_{k-1}^{\text{enc}}, \tau_k)$\; % \tcp*{Upsample coarser features}
            $\hat{\mathbf{Z}}_k^{\text{enc}} \gets \operatorname{ConvBlock}(\tilde{\mathbf{Z}}_k)$\; % \tcp*{Predict finer features}
            $\mathbf{F}_k^{\text{enc}} \gets \mathbf{Z}_k^{\text{enc}} - \hat{\mathbf{Z}}_k^{\text{enc}}$\; % \tcp*{Residual computation}
        }
        $\boldsymbol{R} \gets \boldsymbol{R} \cup \text{lookup}(\mathcal{Q}, \mathbf{F}_k^{\text{enc}})$\; % \tcp*{Quantize and store}
    }
    
    \KwResult{Multi-scale tokens $\boldsymbol{R}$}
\end{algorithm}

\begin{algorithm}[tb]
    \caption{Multi-scale VQ-VAE Reconstruction}
    \label{alg:recon}
    \SetKwInOut{KwData}{Inputs}
    \SetKwInOut{KwIn}{Hparams}
    \SetKwInOut{KwResult}{Return}
    \KwData{Multi-scale tokens $\boldsymbol{R}$}
    \KwIn{Number of scales $K$, scales $\{(s_k, \tau_k)\}_{k=1}^{K}$, codebook $\mathcal{Q}$}
    
    $\mathbf{r}_1 \gets \text{quene\_pop}(\boldsymbol{R})$\;
    $\mathbf{F}_1^{\text{dec}} \gets \operatorname{Lookup}(\mathcal{Q}, \mathbf{r}_1)$\;
    $\mathbf{Z}_1^{\text{dec}} \gets \mathbf{F}_1^{\text{dec}}$\; % \tcp*{Initialize with coarsest-scale features}
    
    \For{$k = 1$ \KwTo $K$}{
        $\mathbf{r}_k \gets \text{quene\_pop}(\boldsymbol{R})$\;
        $\mathbf{F}_k^{\text{dec}} \gets \operatorname{Lookup}(\mathcal{Q}, \mathbf{r}_k)$\; % \tcp*{Retrieve residual features}
        $\tilde{\mathbf{Z}}_k \gets \operatorname{Interpolate}(\mathbf{Z}_{k-1}^{\text{dec}}, \tau_k)$\; % \tcp*{Upsample previous scale}
        $\hat{\mathbf{Z}}_k^{\text{dec}} \gets \operatorname{ConvBlock}(\tilde{\mathbf{Z}}_k)$\; % \tcp*{Refine interpolated features}
        $\mathbf{Z}_k^{\text{dec}} \gets \hat{\mathbf{Z}}_k^{\text{dec}} + \mathbf{F}_k^{\text{dec}}$\; % \tcp*{Fuse prediction with residual}
    }
    
    $\hat{\mathcal{J}} = \operatorname{TrajDecoder}(\mathbf{Z}_{K}^{\text{dec}})$\;
    \KwResult{Reconstructed trajectory $\hat{\mathcal{J}}$}
\end{algorithm}


\begin{algorithm}[htb]
    \caption{Multi-scale Trajectory Generation via STAR-Transformer}
    \label{alg:m-star}
    \SetKwInOut{KwData}{Inputs}
    \SetKwInOut{KwIn}{Hparams}
    \SetKwInOut{KwResult}{Output}
    \KwData{User movement attributes $\mathbf{c}_i$ (home location, commute, etc.)}
    \KwIn{Number of scales $K$, scales $\{(s_k, \tau_k)\}_{k=1}^{K}$, codebook $\mathcal{Q}$}
    
    \tcc{Generate coarsest-scale tokens}
    $\mathbf{r}_1 \gets \operatorname{STAR-Transformer}(\mathbf{c}_i )$\; % \tcp*{Generate initial scale tokens}
    $\mathbf{F}_1 \gets \operatorname{Lookup}(\mathcal{Q}, \mathbf{r}_1)$\; % \tcp*{Retrieve residual features}
    $\mathbf{Z}_1  \gets \mathbf{F}_1$\; % \tcp*{Coarsest-scale representation}
    
    \tcc{Autoregressive next-scale generation}
    \For{$k = 1$ \KwTo $K$}{
        $\tilde{\mathbf{Z}}_k \gets \operatorname{Interpolate}(\mathbf{Z}_{k-1} , \tau_k)$\; % \tcp*{Upsample previous scale}
        $\hat{\mathbf{Z}}_k \gets \operatorname{ConvBlock}(\tilde{\mathbf{Z}}_k)$\; % \tcp*{Predict fine-scale features}
        
        $\mathbf{\hat{r}}_k \gets \operatorname{STAR-Transformer}(\hat{\mathbf{Z}}_k, \mathbf{c}_i )$\; % \tcp*{Generate next-scale tokens}
        $\mathbf{F}_k \gets \operatorname{Lookup}(\mathcal{Q}, \mathbf{\hat{r}}_k)$\; % \tcp*{Retrieve residual features}
        $\mathbf{Z}_k \gets \hat{\mathbf{Z}}_k + \mathbf{F}_k$\; % \tcp*{Fuse prediction and residual}
    }
    
    $\hat{\mathcal{J}} = \operatorname{TrajDecoder}(\mathbf{Z}_{K})$\; % \tcp*{Generate final trajectory}
    
    \KwResult{Generated trajectory $\hat{\mathcal{J}}$}
\end{algorithm}
